Which Imputation Fits Which Feature Selection Method? A Survey-Based Simulation Study

Tree-based learning methods such as Random Forest and XGBoost are still the gold-standard prediction methods for tabular data. Feature importance measures are usually considered for feature selection as well as to assess the effect of features on the outcome variables in the model. This also applies to survey data, which are frequently encountered in the social sciences and official statistics. These types of datasets often present the challenge of missing values. The typical solution is to impute the missing data before applying the learning method. However, given the large number of possible imputation methods available, the question arises as to which should be chosen to achieve the 'best' reflection of feature importance and feature selection in subsequent analyses. In the present paper, we investigate this question in a survey-based simulation study for eight state-of-the art imputation methods and three learners. The imputation methods comprise listwise deletion, three MICE options, four \texttt{missRanger} options as well as the recently proposed mixGBoost imputation approach. As learners, we consider the two most common tree-based methods, Random Forest and XGBoost, and an interpretable linear model with regularization.

==> Outtakes.tex <==

\iffalse
\subsection{Notation}
\label{ssec:notation}

Based on the proposed notation by \cite{vanBuuren2018} and adapted to the regression setup object of this work, let $\mathcal{D}=(X,Y)$ be the dataset with $i = 1, 2, ..., n$ observations, where $X = \{x_{ij}\}$ is the $n \times p$ matrix of $j = 1, 2, ..., p$ independent variables (also can be named \textrm{predictors} or \textrm{features}) and with $Y=\{ y_i \}$ being the $n$-vector for the dependent (predicted) variable in a regression setup. Now, depending on the approach, the dataset can also have some other notations which are:
\begin{itemize}
	\item \textbf{Column-wise:} The variable/feature $j$ in $X$ can be denoted as $X_j$ by dropping the row indicator $i$. 
	\item \textbf{Row-wise:} The observation/unit $i$ in $\mathcal{D}=\{ \langle x_{ij}, y_i \rangle \}$ can be denoted as the tuple $\langle x_{i}, y_i \rangle$ by dropping the column indicator $j$ and then, following this, each observation in $X$ can also be denoted as $\langle x_{i} \rangle$.
	\item \textbf{Element-wise:} $x_{ij}$ is the value of variable/feature $j$ for the $i$-th observation/unit while $y_i$ is then the value of the target/predicted variable in position $i$.
	\item \textbf{Subsets from matrices/datasets:}  a subset of $X$ could be denoted as $X_{subset}$ and if it is also required to be reviewed per column, the notation $X_{subset,j}$ will be referring to the column or feature $j$ of $X_{subset}$ and similarly $\langle x_{subset,i} \rangle$ would make reference to the row or unit $i$ of $X_{subset}$.
\end{itemize}

Now let $R = \{r_{ij}\}$ with $i$ and $j$ as defined for $X$, be the \textrm{response indicator} $n \times p$ matrix denoting whether a value in $X$ is observed. If $x_{ij}$ is observed, then the corresponding entry in R with the same $i$ and $j$ will have a value of 1 ($r_{ij}=1$) and conversely if $x_{ij}$ is missing or not observed: $r_{ij} = 0$. Then, the collections (subsets) of observed and missing data can be defined correspondingly as: 
\begin{equation}
	X_{obs} = \{ x_{ij} \in X  ~|~  r_{ij} = 1 \in R \} \; \text{ and } \; X_{mis} = \{ x_{ij} \in X ~|~ r_{ij} = 0 \in R \}.
\end{equation}
And then, $X = (X_{obs}, X_{mis})$ is the whole dataset \citep[p. ~35]{vanBuuren2018}. 

It is important to mention that there will be no need to define any notation for missing data in the predicted variable $Y$ as along this work it was only of interest to investigate the effect of missing data in the predictor variables.
\\

\subsection{Missing Data Mechanisms}

% Nur eine kurze Erklärung was MCAR, MAR und MNAR ist und warum wir MAR verwenden.

\cite{little2019statistical} define missing data as \textit{"unobserved values that would be meaningful for analysis if observed"}. Then, from this point of view it is of interest the estimation of these values that have not been seen and in that same direction, to perform correct imputations and further analyses depending on the goal of the exercise. But, for this it is first needed to understand the mechanism leading to such missingness.

The theory of \cite{rubin1976inference} formalised the assignment of a probability distribution to the \textrm{response indicators} $r_{ij}$. Following the notation proposed by \cite{vanBuuren2018},  when $\psi$ is the governing vector parameter of the missingness mechanism and the data $X$ is composed by $X_{obs}$ and $X_{mis}$, the model can be expressed as: 
\begin{equation} \label{eq:mismodel}
	\mathbf{P}(R ~|~X_{obs},X_{mis}, \psi).
\end{equation}
And following this, it is possible to define the 3 categories of missing data:
\begin{itemize}
	\item \textbf{Missing completely at random (MCAR):} In this case the probability of being missing is the same for all cases or, in other words, the missingness is not dependent on the data: neither the observed nor the unobserved. Or in mathematical terms:
	\begin{equation} \label{eq:mcar}
		\mathbf{P}(R = 0~|~X_{obs},X_{mis}, \psi)=\mathbf{P}(R=0 ~|~\psi).
	\end{equation}
	\item \textbf{Missing at random (MAR):} Under this, the probability of being missing is the same only withing groups defined by the observed data $X_{obs}$. So:
	\begin{equation} \label{eq:mar}
		\mathbf{P}(R=0 ~|~X_{obs},X_{mis}, \psi)=\mathbf{P}(R=0 ~|~X_{obs},\psi).
	\end{equation}
	\item \textbf{Missing not at random (MNAR):} In this last situation, the probability of being missing varies for unknown reasons and could be expressed as:
	\begin{equation} \label{eq:mnar}
		\mathbf{P}(R=0 ~|~X_{obs},X_{mis}, \psi).
	\end{equation}
\end{itemize}
\noindent For example, if a survey respondent accidentally misses a question or a sensor runs out of battery and can't register measurements because of that, then both are said to be MCAR and $X_{obs}$ is then a simple random sample from $X$ and thus still representative. An example of MAR can occur in a veterinary practice: if the scales need at least 2 seconds to measure the weight of a dog and it is known that some \textrm{border collies} do not manage to sit still for that time, then if the breed is registered for all dogs, the missing data on weight is then MAR (the missingness will depend on the breed). And finally, if people earning very high salaries are more prone to avoid revealing their income when compared to people with regular salaries, then the missing entries are MNAR. In the last 2 cases: MAR and MNAR, the $X_{obs}$ will have biased information in terms of the dogs' weights for the MAR case and the respondents' income for the MNAR case as the resulting samples are not representative of their respective full data $X$ \citep{van2020rebutting}. 


Let's start now by describing the methods and measures used for prediction. Following the notation introduced in Section \ref{ssec:notation}, let $\mathcal{D} = (X,Y)$ be the dataset containing the answers of $n$ respondents . Also, for this section, let them be completely observed, that is: the data has no missing entries. Thus, and just for clarity, as we have all the information from the Target Variable ($Y$) along this report we will always be in a framework of \textrm{Supervised Learning}.

Now and just for this section, let $\mathcal{D}_{train} = (X_{train},Y_{train}) \in \mathcal{D}$ be the subset with $\langle x_{vj},y_v \rangle$ entries where $v  = 1, 2,...,n_{train}$ is the number of entries used to train a model, each $\langle x_{vj},y_v \rangle$ with $j=1,2,...,p$ variables (age, gender, etc..) and with $y_v$ corresponding to the income for such person/observation. Also let $\mathcal{D}_{test}$ with $\langle x_{wj} \rangle$ entries where $w  = 1, 2,...,n_{test}$ be the set of people each with $x_{wj}$ with $j=1,2,...,p$ observed features but for whom the salary is temporarily removed. So, as initially $\mathcal{D}_{test}$ has no salary information, we will need to find a way to train a Model able to predict the person's salary according to the observed features $\langle x_{wj} \rangle$. This predicted income will be denoted as $\hat{y}_w$. 

For simplicity and following the fact that both $\langle x_{vj} \rangle \in \mathcal{D}_{train}$ and $\langle x_{wj} \rangle \in \mathcal{D}_{test}$ have the same number of features $p$, from now on the subscript $j$ will be dropped from the notation (unless needed for further illustration) and the set of observations from the first set (training) will be denoted as $X$ and the set of observations from the second (test) set as $X^*$. So, just to be fully precise: $X = \langle x_{vj} \rangle = \langle x_{v} \rangle\in \mathcal{D}_{train}$ and $X^* = \langle x_{wj} \rangle = \langle x_{w} \rangle \in \mathcal{D}_{test}$.
\\




\subsection{Metrics and Techniques}

Before starting to explain the Statistical Methods and Algorithms used for prediction or classification, lets define some ways to measure how good the models are, how to choose the best one among them and how to compare their results:

\subsubsection{Loss-Function: Mean Squared Error}

In a supervised learning setup for Regression, the main goal is to train a model able to correctly predict a continuous feature. Then, the model will be considered good if it is able to predict exactly the salary of someone from the values observed in the predictors. That is, in a perfect scenario where the prediction for the $i$-th entry is perfect: $\hat{y_i} = y_i$ and then the difference between these 2 values will be $\hat{y_i} - y_i = 0$.

In this sense, a common measure is the \textrm{mean squared error (MSE)}. Able to capture how close a prediction ($\hat{y_i})$ is to the true response $y_i$ it is defined for any $n$ observations as:
\begin{equation}
	\label{eq:mse}
	MSE = \frac{\sum_{i=1}^n (y_i - \hat{f}(\langle x_i \rangle))^2}{n}
\end{equation}
where $\hat{y_i} = \hat{f}(x_i)$ is the prediction of model $\hat{f}$ for the $i$-th observation $\langle x_i \rangle$ and the true value for this observation is $y_i$. So, in that way, the MSE will be small when the predictions are close to the true values and big if they differ from each other \citep[p. ~28]{james2023introduction}.

\subsubsection{Cross-Validation}

As sometimes the available information for training a model could be limited (in other words: small), the model trained could end up providing noisy predictions. As a solution to it, \textrm{cross-validation} is a technique in which the training set is partitioned into smaller groups of data for training the models and then evaluate the results in an repetitive fashion. When the original dataset is split into $\mathtt{k}$ groups, then the process is named $\mathtt{k}$\texttt{-fold cross-validation} \citep[p. ~33]{bishop2006pattern}.

The detailed process is illustrated in Figure \ref{fig:kfold} and made as follows: A dataset $\mathcal{D}$ of $n$ entries is divided into $\mathtt{k}$ disjoint groups (In this case $k=5$). In the first iteration (first colored row in the illustration), $\mathcal{D}_{train}$ (denoted in blue color) is used for training a first model $\mathcal{M}_1$ and its performance then evaluated by plugging in $\mathcal{D}_{test}$ (denoted in orange color in Fig. \ref{fig:kfold}) into $\mathcal{M}_1$ and storing the evaluation metric as $\epsilon_1$. 
\begin{figure}[H]
	\centering
	\caption{k-fold cross-validation. Taken from: \citep[p.  ~203]{james2023introduction}}
	\label{fig:kfold}
	\includegraphics[width = 0.5\textwidth]{Pictures/kfold.png}
\end{figure}

\noindent Then, this process is repeated $\mathtt{k}=5$ times but always changing $\mathcal{D}_{train}$ and $\mathcal{D}_{test}$ until all the groups are used once as the test subset for evaluation (note how the red groups are changing row-wise in the Figure) and all the combinations of the other sets in blue are used as training subsets for each model trained in each iteration. In the end, after computing all the $\mathtt{k}=5$ evaluation metrics, the final cross-validation score is simply computed as the average of these epsilons. So, in general, the cross-validated error (or any other evaluation metric) can be written as follows:
\begin{equation}
	CV_\texttt{k} = \frac{1}{\texttt{k}} \sum_{i=1}^{\texttt{k}} \epsilon_i
\end{equation}

In general, Machine Learning Algorithms have \textrm{parameters} and \textrm{hyperparameters} needed to make them work. \textrm{Parameters} are for example in a classic linear model, the linear model coefficients $\beta$ belonging to the data and which are obtained after training the model. So, recalling the notation from the last section, and precisely as presented in Equation \eqref{eq:governors}, the parameters $\theta$ that are governing $X$. \textrm{Hyperparameters}, on the other hand, are variables configured by the practitioner or the user training the model in order to determine the fitness of the parameters to the data. But then, as these last ones are defined by the practitioner, the process of finding the optimal combination of them improving a machine learning for a given task is known as \textrm{hyperparameter optimization (HPO)} and the process is also known as  \textrm{model tuning}. Basically, as there is no closed-form solution to find the best hyperparameters, each of the possible combinations are used to train a machine learning algorithm. Then, all are evaluated with the same Loss-Function and finally the model with the best performance is chosen as the final winner to be used for predictions \citep[p. ~81]{Bischl2024}. 

In light of this, the major disadvantage of \textrm{cross-validation} is that, when used with computationally expensive models, the final time to run the whole solution is increased by a factor of $\mathtt{k}$. And even more, when the scientist performing the model training is also doing \textrm{hyperparameters optimization (HPO)}, as the computational time might increase exponentially \citep[p. ~33]{bishop2006pattern}. 

\subsubsection{Nested Resampling}

In Machine Learning, the \textrm{Bias-Variance trade-off} describes the relationship between the following 3 errors: first \textrm{bias}, being the difference obtained after modifying the complexity of a model by for example, reducing the number of parameters in a linear model from 10 variables to 5 being used to predict $Y$. The second one, \textrm{variance}, is the amount of change in the estimations (or predictions $\hat{y}_i$) made by the model in presence of a different dataset which, ideally should not vary much. And the third one is the \textrm{test set MSE}, which understood as in Equation \eqref{eq:mse} is the metric of how good a prediction of certain model is in terms of its distance to the true value. In general, as the bias is reduced by for example increasing the degree of a polynomial model and fitting better to the data in a process known as \textrm{overfitting}, its variance will be increased as the model will not be able to fit well to new data. Thus, the goal will be to find a model capable of dealing which such trade-off and in which both variance and bias are low \citep[p. ~34]{james2023introduction}. 

When performing HPO, it is needed to reduce the bias when estimating how good a model performs. Given that using the same $\mathcal{D}_{train}$ to find the best combination of parameters and to evaluate as well the performance of a model it might end up being biased. For this, \textrm{nested resampling} adds another sampling level to the regular Cross-Validation in order to separate the model optimization (HPO) from the process of estimating the performance of the tuned model. 

\noindent The process of nested resampling is shown in Figure \ref{fig:nestedres} for an outer resampling with 3 folds and inner resampling of 4 folds and is as follows: The whole dataset is split into 3 outer folds 2 $\mathcal{D}_{train-out}$ in light blue  and one $\mathcal{D}_{test-out}$ denoted in green is saved for later evaluation. Then, the 2 training sets are split into 4 inner folds $\mathcal{D}_{inner}$ as shown with dark blue colors. On them, HPO is performed and tuned by iterating the test fold as shown in blue for the 4 inner folds. And then, the best configuration $\hat{\lambda}$ is stored. Done that, these best parameters from $\hat{\lambda}$ are used for training a new model with $\mathcal{D}_{train-out}$ but evaluated by measuring its prediction error in $\mathcal{D}_{test-out}$. The process is repeated then for all outer loops (that is by iterating and exchanging the green square into the other 2 folds) to finally aggregate all the prediction errors and compute the final overall performance measure \citep{bischl2023hyperparameter}. 

\begin{figure}[H]
	\centering
	\caption{Nested Resampling for one iteration in the outer folds. Adapted from: \cite{bischl2023hyperparameter}}
	\label{fig:nestedres}
	\includegraphics[width = 0.7\textwidth]{Pictures/Nested.png}
\end{figure}

\fi 

\iffalse


\subsection{Lasso Regularized Linear Models}

Starting from the usual linear regression model, the prediction for an observation $i$ from $\mathcal{D}$, is defined to be: 
\begin{equation}
	\begin{split}
	\hat{y}_i & = \beta_0 + x_{i1} \beta_1 + ... + x_{ip} \beta_p \\
					&= \beta_0 + \sum_{j=1}^p x_{ij} \beta_j,
	\end{split}
\end{equation}
where the coefficients $\beta_j$, when obtained by the ordinary least squares (OLS) method, are chosen such that they minimize:
\begin{equation}
	\label{eq:RSS}
	\begin{split}
	RSS & = \sum_{i=1}^n (y_i - \hat{y_i})^2 \\
			& = \sum_{i=1}^n (y_i - \beta_0 - \sum_{j=1}^p x_{ij} \beta_j)^2,
	\end{split}
\end{equation}
which is the \textrm{Residual Sum of Squares (RSS)} defined to be the sum of the squared differences between the predicted values $\hat{y_i}$ and the true observed values $y_i$ \citep[p. ~71]{james2023introduction}.

However, sometimes the OLS results might have low bias and large variance being suitable to be improved by setting some coefficients $\beta$ to 0. In that way, the variance is decreased at the expense of more bias ending in an overall prediction accuracy improvement together with a more interpretable result as the final model after discarding some features will have less predictors which will be the ones exhibiting the strongest effects. A technique combining both interpretation and accuracy is the \textrm{lasso}: least absolute shrinkage and selection operator \citep{tibshirani1996regression}. 

Working similarly to the OLS, the coefficients in Lasso are found to be the ones minimizing the quantity:

\begin{equation}
	\label{eq:lasso}
	\sum_{i=1}^n (y_i - \beta_0 - \sum_{j=1}^p x_{ij} \beta_j)^2 + \lambda \sum_{j=1}^p | \beta_j |,
\end{equation}
where the first term is RSS as in Equation \eqref{eq:RSS} and the second term introduces a penalty term which, depending on the value of the penalization parameter $\lambda \neq 0$ will start to shrink the coefficients to 0, performing \textit{variable selection}. Extreme values for $\lambda$ are: when chosen to be 0, will be the case of the classic OLS as the penalization term is removed or if $\lambda = \infty$  then all the coefficients $\beta_j$ will be shrinked to 0. In the end, the selection of the value for $\lambda$ is commonly made by cross-validation methods trying to find the value leading to the lowest errors \citep[p. ~244]{james2023introduction}. 
\\ 

\subsection{Decision Trees and Random Forests}

Decision Trees are Machine Learning algorithms for both Regression and Classification tasks. They try to learn from the data by segmenting the features spaces into regions. For example, imagine the Foreigner's Office in Germany would like to develop a model to evaluate if the someone's income will be above a threshold of 4,000 EUR per month to be eligible for a special Residence Permit. Thus, if one of the $p$ features of $X$ used as predictor in the model is the work experience (\textit{workexp}) and there would exist an evident salary gap for people with less than one year of experience, then the feature space while the model is trained could be split into 2 regions denoted as: $\mathcal{R}_1 = \{\langle x_{ij},y_i \rangle ~|~ \textit{workexp} < 1\}$ and $\mathcal{R}_2 = \{\langle x_{ij},y_i \rangle ~|~ \textit{workexp} \geq 1\}$ and then, all the respondents from $\mathcal{R}_1$ would have lower salaries than the ones in $\mathcal{R}_2$. That is, any salary $y_1 = \{ y_i ~|~ \langle x_{ij},y_i \rangle \in \mathcal{R}_1 \} $ will be lower than any $y_2 = \{ y_i ~|~ \langle x_{ij},y_i \rangle \in \mathcal{R}_2 \}$.

\usetikzlibrary{shapes.geometric}

\begin{figure}
	\centering
	\caption{Decision Tree Example}
	\label{fig:dtree}
	\begin{tikzpicture}[
		grow = down,
		sibling distance = 10 em,
		level distance = 5 em,
		edge from parent/.style = {draw, -latex}
		]
		%Tree
		\node [draw]{\textbf{\textit{workexp}}}
		child { node {2000} edge from parent node [fill = white, text = gray, font = \small] {<1} }
		child { node [draw] {\textbf{\textit{gender}}}  
			child { node {3800} edge from parent node [fill = white, text = gray, font = \small] {female}}
			child { node {4100}	edge from parent node [fill = white, text = gray, font = \small] {male}}
			edge from parent node [fill = white, text = gray, font = \small] {$\geq$ 1}};
	\end{tikzpicture}
\end{figure}

\noindent Now, if there would be a case in which another condition is found for the salary to change depending on the value of the observation, for example the \textit{gender}, then one Decision Tree (under this example) would be as shown in Figure \ref{fig:dtree}. From it, \textit{workexp} and \textit{gender} are the only features needed to predict the expected salary for someone from whom we would have information regarding the years of experience and the gender. 

Furthermore, this decision tree would be said to have: 3 \textrm{leaves} or \textrm{terminal nodes}: one per region among these 3 (each being a salary) from left to right in the image. So, explicitly: the first node is $2000 = \{y_i \in \mathcal{R}_1  ~|~ \textit{workexp} < 1\}$, the second one $3800 = \{y_i \in \mathcal{R}_2 ~|~ \textit{workexp} \geq 1, \textit{gender} = female\}$ and the third one $4100 = \{y_i \in \mathcal{R}_3 ~|~ \textit{workexp} \geq 1, \textit{gender} = male\}$. Which leads to the tree with \textrm{depth} of 2 levels: one for the \textit{workexp} and another one for the \textit{gender}.

With this explained, it is now time to get into the process of building a decision tree. \cite{james2023introduction} would summarize it in 2 general steps:
\begin{enumerate}
	\item Divide the feature space $X$ into $K$ distinct and disjoint regions: $\mathcal{R}_k$, with $k = 1, 2, ..., K$.
	\item For every new observation $\langle \ddot{x}_{ij}, \ddot{y}_i \rangle$ falling in $R_k$, the same prediction $\hat{\ddot{y}}$ is made for the whole region. 
\end{enumerate}

So, in a regression setup, it would be possible to simply predict the \textrm{mean} of the observations in region $\mathcal{R}_k$ where $\langle \ddot{x}_i \rangle$ belongs. Or, in a classification setup, it will be desired to simply predict the \textrm{most common class} in the region $\mathcal{R}_k$ where $\langle \ddot{x}_i \rangle$ belongs. In other words, $\hat{\ddot{y}}$ will be the $y_i$ with the highest number of ocurrences in $\mathcal{R}_k$ when $y_i$ would not be the salary but perhaps an already encoded variable mapping to "yes" if the salary is above 4000 EUR and "no" for any other case. 

But then, how is the feature space divided into regions? The answer is described in Algorithm \ref{alg:tree}. First, it is needed to find the best variable $X_j$ to divide the data in the first split. For this, a metric is needed to make such decision which depending on the setup are the following:
\begin{itemize}
	\item \textbf{Regression:} The most common one is the RSS as defined in Equation \eqref{eq:RSS} and adapted to find the Regions $\mathcal{R}_k$ minimizing this formula: 
	\begin{equation}
		\label{eq:RSStree}
		RSS =  \sum_{k=1}^K \sum_{i \in \mathcal{R}_k} (y_i - \hat{y}_{\mathcal{R}_k})^2,
	\end{equation}
	where $\hat{y}_{\mathcal{R}_k}$ is the predicted mean of the observed values in $\mathcal{R}_k$.
	\item \textbf{Classification:} The \textbf{Gini Index}, defined for the $k$-th region as:
				\begin{equation}
						G_k = \sum_c^\mathcal{C} \hat{p}_{kc} (1-\hat{p}_{kc}),
				\end{equation}
		where $c = 1,...,\mathcal{C}$ is the number of classes available (categories or labels, which for a binary case will be $\mathcal{C}=2$)  and $\hat{p}_{kc}$ is the proportion of observations of class $c$ in the $k$-th region. It is worth saying that, this index is also known as a measure of \texttt{purity} as the closer it gets to $G_k = 0$, the more pure the node is because $\hat{p}_{kc}$ is also closer to 0 or 1, meaning that the observations in the node are (almost) all from the same class \citep[p.  ~338]{james2023introduction}. And additionally, the predicted label for each region will be the most common one in it.
\end{itemize}
\noindent 

\begin{algorithm}[!h]
	\caption{Decision Tree, adapted from \citep[p. ~333-338]{james2023introduction}}
	\label{alg:tree}
	\begin{algorithmic}[1]
		\Require $\mathcal{D} = \langle x_{ip},y_i \rangle$ = dataset with target variable.
		\Require $n^*$ = desired number of observations in each terminal node or region.
		\Require $F$ = desired number of folds to split $\mathcal{D}$ into for Cross-Validation.
		\State $\mathcal{P} = {X_1,X_2,...,X_p}$, list of features in $\mathcal{D}$
		\While {number of observations in the terminal nodes is more than $n^*$ or $\mathcal{P} \neq \emptyset$}
		\State choose the $X_i$ leading to the lowest \textbf{RSS} (Regression) or \textbf{Gini Index} (Classification) when dividing the feature space into 2 regions: $\mathcal{R}^1_{i}$ and $\mathcal{R}^2_{i}$.
		\State store the resulting regions.
		\State remove $X_i$ from $\mathcal{P}$.
		\EndWhile
		\State store the tree $T_0$
		\State perform cost complexity pruning on $T_0$ and get all the best possible sub-trees as a function of $\alpha$.
		\State Split $\mathcal{D}$ into $F$-folds
		\For{$f = 1,2,...F$}
		\State repeat steps 1 to 8 on all but the $f$-th fold.
		\State evaluate the prediction error on the $f$-th fold as a function of $\alpha$.
		\State average the results for each value of $\alpha$
		\State choose the value of $\alpha$ that minimizes the average error
		\EndFor
		\State return the subtree from 8 that corresponds to the chosen best $\alpha$ in Step 14. 
	\end{algorithmic}
\end{algorithm}

So, after the parameter $X_j$ leading to the smallest RSS or Gini Index is found (depending on the task), the split is made, the regions are created and then the process continues iteratively for the remaining features until a desired minimum number of observations per node is reached or until there are no more features to keep splitting the data.

Done this, as the resulting tree $T_0$ will be very likely a large one overfitted to the data, a process named \textrm{cost complexity pruning} is followed (step 8 in Algorithm \ref{alg:tree}): The idea is to find a smaller tree $T \subseteq T_0$ able to minimize the prediction error by the introduction of a tuning parameter $\alpha$ (taking non-negative values) that penalizes the number of terminal nodes in $T$ (denoted as $|T|$). So, in the end, the goal is to minimize the following equation:
\begin{equation}
	\label{eq:eqTrees}
	\sum_{k=1}^{|T|} \; \sum_{i: \langle x_i \rangle \in \mathcal{R}_k} \big( y_i - \hat{y}_{\mathcal{R}_k}\big) + \alpha |T|,
\end{equation}
where, $k = 1,2,...,K$ is the number of regions of $T$, $\langle x_i \rangle \in \mathcal{R}_k$ are the observations in region $k$, $y_i$ is the observed value or label corresponding to each of the $\langle x_i \rangle $ observations and $\hat{y}_{\mathcal{R}_k}$ being the predicted value or label for the tree $T$ in the $k$-th region \citep[p.  ~336]{james2023introduction}. 

Then, when $\alpha=0$ the resulting tree should be $T_0$ (the largest, overfitted, unpruned tree with the lowest RSS) but as long as it increases, branches of the tree will be pruned and for each value of $\alpha$ will exist a tree $T$ being as small as possible. In the end, the value of $\alpha$ is chosen via cross-validation and the corresponding tree is returned as shown in steps 9 to 16 in Algorithm \ref{alg:tree} \citep[p.  ~337]{james2023introduction}.

Decision trees are popular because they are easy to explain and even graphically displayed. Furthermore, because of their ability to deal with both numerical (quantitative) and categorical (qualitative) features. However, they can be non-robust as a small change in data can cause very different predicted results \citep[p.  ~340]{james2023introduction}. 

\subsubsection{Random Forests}
\label{ssec:rf}

The main idea behind the Random Forests is to train many trees that in the end will be used to do predictions that are averaged to get a single final value when in a Regression task or just as in the case of a Classification task in a Decision Tree setup, the \textrm{most common} predicted class will be the final one chosen for $\hat{y_i}$. This last method is also known as \textrm{majority vote} \citep[p. ~344]{james2023introduction}.

One big improvement Random Forests have compared to Decision Trees is the variance reduction. Based on the fact that the average of a sample will have lower variance than the observations' variance, the basis of the mechanism can be seen directly: let $Z_1, Z_2, ..., Z_n$ be a set of $n$ independent random variables with variance $\sigma^2$, then its mean $\bar{Z} = \frac{1}{n} \sum_{i:1}^n Z_i$ will have variance of $\sigma^2/n$. Thus, translating this concept to the Trees' scenario: it will be useful to have many different training sets from the population so it is possible to train many different trees with high variance predictions that then will be averaged (for a regression setup or a majority vote for a classification task could also be performed) to get a single prediction value with low variance \citep[p. ~343]{james2023introduction}.

The Random Forest process is described in Algorithm \ref{alg:rf}: first it is needed to generate $B$ training sets, however, as it might not be possible to get all that many sets when the dataset is small, the solution is to perform \textrm{Bootstrap aggregation} or \textrm{bagging}. That is, take repeated samples from the observations available in $\mathcal{D}$ until generating $B$ training sets $\mathcal{D}_b$ with $b=1,2,...,B$ \citep[p. ~343]{james2023introduction}. 

\begin{algorithm}[!h]
	\caption{Random Forests' algorithm, adapted from \citep[p. ~343-347]{james2023introduction}}\label{alg:rf}
	\begin{algorithmic}[1]
		\Require $\mathcal{D}= \langle x_{ip},y_i \rangle$ = dataset with target variable.
		\Require B: number of trees desired to be trained
		\State $\mathcal{Y} = \emptyset$
		\For{b = 1,2,..., B}
		\State randomly generate $\mathcal{P}^*$ with size $\sqrt{p}$.
		\State generate a Bootstrapped dataset $\mathcal{D}_b$
		\State train a decorrelated Decision Tree $T_b$ as in Algorithm \ref{alg:tree} using the chosen features $\mathcal{P}^*$ from $\mathcal{D}_b$
		\State predict $\hat{y}^*$ using $T_b$
		\State store $\hat{y}^*$ in $\mathcal{Y}$
		\EndFor
		\State return the final predicted $\hat{y}$: the average of $\mathcal{Y}$ in a regression setup or the most common predicted class of $\mathcal{Y}$ in a classification task. 
	\end{algorithmic}
\end{algorithm}

Done that, for each of the recently obtained sets $\mathcal{D}_b$, train a \textrm{decorrelated} Tree. That is, a tree for which only a random sample (a subset) of all the possible $p$ features of $X_b$ is used when deciding the splits: so, $\mathcal{P}$ from Algorithm \ref{alg:tree} becomes now $\mathcal{P}^*$ and has less than $p$ available variables to choose from when building the tree: $|\mathcal{P}^*| < |\mathcal{P}|$. The size of this subset of features is commonly chosen to be $|\mathcal{P}^*| \approx \sqrt{p}$. 

This last step ensures all the features $p$ will have more chance to be considered for the splits, even the ones with low Gini Index, granting a wide variety of trained trees leading to a more reliable final prediction which also has low variance after the majority vote principle is applied when in Classification Tasks. \citep[p. ~347]{james2023introduction}. 

Additional to this, another advantage of the Random Forests is that using a large value of $B$ will not lead to overfitting, so it is common to use a large value of bootstrapped samples to make sure the error is reduced. However, the cost of such procedure is that the interpretability from the Decision Trees is lost after all the iterations: there is no way to trace back how the decisions are made for the final predictions \citep[p. ~347]{james2023introduction}.

In any case, after all the training procedures are resulting into many Decision Trees, Random Forests allow to measure the importance of each feature $p_i \in p$ for the final predictions among all the trees used in the model, being very useful for space reductions that might be used to discard features that are not relevant for generating predictions (\textrm{feature selection}) \citep[p. ~347]{james2023introduction}. In practice, measures like the Gini Index or RSS are employed to account for such importances depending on the task for which the model is being trained. 

One last remark is worth to be made and it is with regards to how Tree-based methods perform in presence of Missing Data. According to \cite{JMLR:v11:ding10a}, a simple and powerful way to impute missing data for binary classification when training Tree-based models is to impute all the missing values with a single large value creating the need of separation of data, implying that any split involving the variable with missing values will put all the imputed values into the same node of the tree. Additionally, \cite{buczak2023analyzing} showed how Random Forests' classification results improved under certain Imputation Methods while \cite{ramosaj2022relation} found that Random-Forest-based prediction intervals (in Regression tasks) are improved in combination with Tree-based imputation methods for missing data.
\\ 

\subsection{XGBoost}

Boosting methods are based on a similar principle to the one from Random Forests. The goal is to train many trees that grouped will improve the accuracy of the predictions made by them. However, there are some variations to it which can be a combination of the following ones \citep[p. ~349]{james2023introduction}: 
\begin{itemize}
	\item the trees are grown \textrm{sequentially} (\textrm{Boosting}): that is, after training the first tree $T_0$ or $f_0(x)$, the next ones are trained using the residuals from the previous one instead of the observations $y_i$. Thus, the areas in which the former $T_{t-1}$ or $f_{t-1}(x)$ trees did not do good predictions are improved iteration after iteration.
	\item each tree is most of the times small.
	\item there is a \textrm{shrinkage parameter} controlling the \textrm{learning rate} of the boosting method. The tinier its value, the bigger $B^*$ (number of boosting trees) will be needed to be in order to provide good predictions while leaving a large value of shrinkage will lead to good results at smaller values of $B^*$. 
\end{itemize}
\noindent  In particular, XGBoost is a Tree Based Machine Learning method which incorporates, among other additions, Gradient Boosting after a combination of the variations listed before. In what is left of this subsection, it is going to be explained how it works according to \cite{chen2016xgboost} and with some adaptations in the notation to follow the one along this report. 

First of all, let $\mathcal{F}$ be the space of regression trees $f_b$ (with $b = 1, ..., B^*$) used to predict $\hat{y_i}$ in an additive way so it can be expressed as: 
\begin{equation}
	\hat{y_i} = \phi(\langle x_i \rangle) = \sum_{b=1}^{B^*} f_b(\langle x_i \rangle), \quad f_b \in \mathcal{F},
\end{equation}
so, the final prediction $\hat{y_i}$ of a new entry $\langle x_i \rangle$ will be the function $\phi (\cdot)$ corresponding to the sum of all the predictions from the $B^*$ trees grown sequentially when evaluated with $\langle x_i \rangle$. Where, each tree structure $q$ maps every entry $\langle x \rangle$ to a leaf index $T = 1, ..., |T|$ so $q(\langle x \rangle) = T$ and $f_b(\langle x \rangle) = w_{q(\langle x \rangle)} = w_T$ is an independent tree structure $q$ with leaf weights $w_{q(\langle x \rangle)}=w_T$. So, in simple terms, $w_T$ denotes the score $w$ of leaf $T$ from tree $f_b(\cdot)$ with structure $q$. 

Once again, the main goal is to minimize an objective function following the same basis as the ones presented in Equation \eqref{eq:lasso} for the Lasso and in Equation \eqref{eq:eqTrees} for Decision trees and Random Forests: find the set of parameters $\gamma$ and $\lambda$ that minimizes a single expression made of a combination between a Loss Function and a Regularization Term accounting for the model's complexity through a penalization parameter. In the case of XGBoost, it is defined to be:
\begin{equation}
	\label{eq:xgboost}
	\mathcal{L (\phi)} \, = \, \underbrace{\sum_{i=1}^n l(\hat{y_i}, y_i) }_\text{Loss} 
									\; + \; \underbrace{\sum_{b = 1}^B ( \gamma |T_b| + \frac{1}{2} \lambda \sum_{j=1}^{|T_b|} w_j^2 )}_\text{Regularization},
\end{equation}
 where the first term is the loss that might be chosen for example to be the MSE in a regression task or the log-loss in a classification task and the second one is a Regularization parameter made of 2 terms: the first one penalizes the size of each tree $|T_b|$ (accounted as the number of leaves in the tree) by means of $\gamma$ and the second one penalizes the score in the leaves $w_j$ with the parameter $\lambda$. Please note that the notation of $\lambda$ is kept for all the ML Models just to denote its nature and behavious as penalization parameter but they are indeed different depending on the model being used. 
 
Now, given that finding the solution that minimizes this equation can't be simply made by traditional optimization methods, the model is then solved by training it in an additive manner. That is, $\hat{y}^{(t)}_i$ (the prediction in iteration $t$) will be the (greedy) sum of the prediction in the previous step $t-1$ and the prediction of the tree $f_t(\cdot)$ that improves the most the model in the current step $t$ for $\langle x_i \rangle$, so: $\hat{y}^{(t)}_i = \hat{y}^{(t-1)}_i + f_t(\langle x_i \rangle)$. And then, replacing this in Equation \eqref{eq:xgboost}, will lead to:
\begin{equation}
	\mathcal{L (\phi)}^{(t)} \, = \, \sum_{i=1}^n l \big(y_i, \hat{y}^{(t-1)}_i + f_t(\langle x_i \rangle)\big) \; + \; \sum_{b = 1}^B \big( \gamma |T_b| + \frac{1}{2} \lambda \sum_{j=1}^{|T_b|} w_j^2 \big).
\end{equation}

Which then, following a second order approximation and rearranging the sums can be reduced to the following expression:
\begin{equation}
	\begin{split}
	\tilde{\mathcal{L}}^{(t)} \, &= \, \sum_{i=1}^n \big[g_i f_t(\langle x_i \rangle) + \frac{1}{2} h_i f_t^2(\langle x_i \rangle) \big] + \; \sum_{b = 1}^B \big( \gamma |T_b| + \frac{1}{2} \lambda \sum_{j=1}^{|T_b|} w_j^2 \big) \\
				&= \, \sum_{j=1}^{|T_b|} \big[ \, \big( \sum_{i \in I_j} g_i\big)w_j \, + \, \frac{1}{2} \big( \sum_{i \in I_j} h_i + \lambda \big)w_j^2 \, \big] + \gamma |T_b|
	\end{split}
\end{equation}
with $g_i = \partial_{\hat{y}^{(t-1)}} l(y_i, \hat{y}^{(t-1)}) $ being the first gradient and $h_i = \partial_{\hat{y}^{(t-1)}}^2 l(y_i, \hat{y}^{(t-1)}) $ the second gradient of the Loss in step $t-1$ and with $I_j = \{ i \, | \, q(\langle x_i \rangle) = j \}$ being the set of entries in leaf $j$.

Now, how is it possible to measure the quality of a tree structure $q$, or in other words, how can we compare the tree structures in order to find the best one? Well, just as the Gini Index for Random Forests and Decision Trees, XGBoost introduces a impurity score to evaluate them. For this, let now $G_j = \sum_{i \in I_j} g_i$ and $H_j = \sum_{i \in I_j} h_i$ be the sums of the first and second order gradients for all the observations in leaf $j$. Then, the optimal weight or score $w_j^*$ for such leaf will be:
\begin{equation}
	w_j^* = -\frac{G_j}{H_j + \lambda},
\end{equation}
and the optimal value for the objective function to be:
\begin{equation}
	\label{eq:impXG}
	\tilde{\mathcal{L}}^{(t)} = -\frac{1}{2} \sum_{j=1}^{|T_b|} \frac{G_j^2}{H_j+\lambda} + \gamma |T_b|.
\end{equation}
However, as in practice it is not possible to evaluate all the possible tree structures $q$, XGBoost uses a greedy algorithm to grow the tree starting from a simple tree with 0 depth and then for each leaf node, measures the gain of a possible split or, in other words, how much the scores improve after a split is made which is nothing else than evaluating Equation \eqref{eq:impXG} in the current node with observations $I$ and the entries in the newly generated leaves after the split denoted as $I_L$ for the left leaf and $I_R$ for the right leaf (please note $I = I_L \cup I_R$) and then, accordingly, the sums of the first and second order gradients in the left and the right leaves $G_L, G_R, H_L$ and $H_R$:
\begin{equation}
	\label{eq:lsplit}
	\mathcal{L}_{split} = \frac{1}{2} \Big[ \frac{G_L^2}{H_L+\lambda} + \frac{G_R^2}{H_R+\lambda} + \frac{(G_L+G_R)^2}{H_L+H_R+\lambda} \Big] - \gamma,
\end{equation}
 and then, it is possible to find the best split (the one leading to the maximum score of this last equation) as shown in Algorithm \ref{alg:splitxg}.
 
 \begin{algorithm}[!h]
 	\caption{Exact Greedy Algorithm for Split Finding, adapted from \citep{chen2016xgboost}}\label{alg:splitxg}
 	\begin{algorithmic}[1]
 		\Require $I$ = observations in the currrent node, sorted. 
		\State Initialize $BestScore=-\infty$.
		\State Initialize $BestSplit=\emptyset$.
 		\State Calculate $G$ and $H$.
 		\For{$j = 1,2,..., p$}
 			\State Initialize $G_L=0$ and $H_L=0$.
 			\For{$i = 1,2,..., |I|$}
 				\State Calculate $G_L = G_L + g_i$
 				\State Calculate $H_L = H_L + h_i$
 				\State Calculate $G_R = G - G_L$
 				\State Calculate $H_R = H - H_L$
 				\State Calculate $Score = \frac{G_L^2}{H_L+\lambda} + \frac{G_R^2}{H_R+\lambda} - \frac{(G_L+G_R)^2}{H_L+H_R+\lambda}$
 				\If {$Score >= BestScore$}
 					\State $BestScore = Score$
 					\State $BestSplit = i,j$
 				\EndIf
 			\EndFor
 		\EndFor
 		\State return $BestSplit$
 	\end{algorithmic}
\end{algorithm}

Additionally, it can be seen from Equation \eqref{eq:lsplit} that it also can be used to prune the tree: by growing a tree to maximum depth and then recursively removing all the leaves where the following condition is met:
\begin{equation}
\frac{G_L^2}{H_L+\lambda} + \frac{G_R^2}{H_R+\lambda} - \frac{(G_L+G_R)^2}{H_L+H_R+\lambda} < \gamma,
\end{equation} 
or, in other words, when the gain from the split is lower than $\gamma$.

Furthermore, measuring $G$ and $H$ at each split and for the many variables in the model as presented in Algorithm \ref{alg:splitxg}, serves as a metric for quality splits which is extendable for feature selection. Equation \eqref{eq:lsplit} can also be seen as the gain after a split is made and then account for a measure of Feature Importance. According to the documentation of the algorithm, the gain is finally presented as the fraction (in percentage) of contribution of each feature to the model with respect to the total gain of this feature for all the splits in which it was involved \citep{chen2019package}. 

So, up until this point has been described how XGBoost works in general. But, there are some more enhancements improving its functionalities that are:
\begin{itemize}
	\item Shrinkage: By adding a parameter $\eta$ accounting the weights of each tree being added in each boosting step. So, in other words, it ends up scaling by a factor of $\eta$ the contribution of each tree $f_t(\cdot)$, $f_{t+1}(\cdot)$, etc. to the final prediction of the whole boosted ensemble. If closer to 0, then smaller is the contribution of each tree and more steps will be needed if compared to a bigger value of $\eta$ which will need less trees to get to the same error value.
	\item Column Subsampling: just as with Random Forests, the trees in XGBoost are constructed with a subsample of all the parameters $p$, reducing as well in this case the over-fitting of the model.
	\item Approximate algorithm for split finding: even though Algorithm \ref{alg:splitxg} is very powerful as it lists all the possible splitting points in a greedy way, in presence of large datasets it could get hard to manage it completely into memory. Then, it is solved by grouping the candidates for the splits into percentiles of the features (also called \textrm{blocks}): in a global variant by setting a set of candidate splits during the initial construction phase of the tree which are re-used in every level or in a local variant refining the set of candidates after each split. 
	\item Sparsity-aware Split Finding: In cases where $X$ is sparse due to missing values or frequent zeros resulting from (for example) one-hot encoding, XGBoost introduces a \textit{default direction} in each tree node so, learned from the data used to train the model, whenever a missing entry shows up it is classified into the default direction. 
	\item Computational Improvements: As mentioned before, the introduction of \textrm{blocks} of data, allow the storage in in-memory units improving the sorting procedures needed for the splits by computing them before training and re-using such blocks in the latter iterations following a linear scan. Additionally, it enables parallelization and in combination with memory-aware mechanisms even allows for computations using disk space in addition to the main memory usage. 
\end{itemize}
\noindent During the last few years, XGBoost and variations of Gradient boosting decision trees have been leading the winners' charts in Machine Learning Competitions. Particularly, XGBoost was in 2015 among the top solutions for contests such as the ones available in Kaggle and KDDCup during 2015 \citep{chen2016xgboost}. 
 \\

\subsection{Feature Importance}
\label{ssec:featsel}

In the last few subsections we have reviewed how the ML algorithms work and their internal mechanisms to perform feature selection: in the lasso case, the value of the penalization parameter $\lambda$ forces some of the coefficients $\beta_j$ to be shrinked to 0 and then leaving some of them as the chosen ones in the final best model (the ones with non-zero values). So, the Lasso algorithm performs feature selection directly.

However, in the case of Random Forests and XGBoost, the algorithms are able to compute a metric accounting for the "importance" of each feature in the trees used in the model being trained. But, the final result will have the list of all the features and their importance value: an accumulated sum of Gini Index for the Random Forests case and the fraction of contribution in Gain for the XGBoost. So, in the end there is no real feature selection but it is still interesting to see how each model accounts the importance of each variable and then compare the results between the models.

Thus, in order to stablish a common ground to compare how good are these Tree-based methods for feature selection, it is needed to define a filter-based Feature Selection. Following the procedure described by \citep{Bischl2024} in its chapter 6.1.4, a threshold is defined in order to choose just the best features from each resulting model and for both XGBoost and Random Forests only the values with Importance measures above or equal to the median value of importance (in their respective units) will be kept for the final comparison of features chosen by these 2 tree-based Machine Learning Methods.

\fi
 

\iffalse
\section{Handling Missing Data}
\label{sec:MissingData}

Following the definition of missing data provided by \cite{little2019statistical}, as there is meaningful information lying under these unobserved data, it is then interesting to investigate some methods to deal with missing data: either by imputing ("filling in" \citep[p. ~4]{little2019statistical}) the dataset in order to make it complete ( to replace missing elements $x_{ij}$ by -hopefully suitable- values) or simply ignore the entries $\langle x_{ij} \rangle$ which might have any unobserved element. 

In this section, we are going to review some of the available methods for dealing with missing data: starting from simple techniques like listwise deletion or naive imputation and then getting into methods of Multiple Imputations to end the chapter with some metrics used to measure the imputation quality. 
\\

\subsection{Listwise deletion}

Also known as \textrm{Complete-case analysis}, this method deletes all the units or observations $\langle x_{ij}, y_i \rangle$ for which there is one or more missing values. That is, in our regression setup with a dataset $\mathcal{D} = (X,Y)$, it removes at the same time all the row $\langle x_{i}\rangle \in X$ and the values $y_i \in Y$ for which there is any $r_{ij}  = 0$. 

The advantages of this approach are the simplicity to implement as there is no need of any modification of the data (nor imputation) and if the data are MCAR, it produces unbiased estimates of means, variances and regression weights, together with correct standard errors and significance levels (however, larger relative to $X$). On the other hand, in some cases the amount of discarded information could be substantial, more when the number of variables $p$ is large \citep{vanBuuren2018}.  Additionally, if the data are not MCAR, the estimates obtained from inferential analysis could be biased even in presence of small missingness rates \citep{van2020rebutting, SchwerterPauly2024}.
\\

%\subsection{Naive Imputation}

%Part of the also known \textrm{Single Imputation Methods}, this method is one simple version of filling-in the unobserved values by replacing them with one plausible value per missing variable. In mathematical terms, if for any feature $X_j$ there is one or more missing entries (at least one value in $R_j$ is 0), any missing entry $x_{ij} \in X_j$ (that is the one with $i$ and $j$ for which $r_{ij}=0$) is replaced by an estimate $\tilde{\theta}_j$ constant and unique for the feature $X_j$. Such estimate $\tilde{\theta}_j$ is usually chosen to be the mean, the median or the mode (most observed value) of the observed values for feature to be imputed $X_{obs,j}$. 

%Just as with the listwise deletion, this method is simple in its implementation but is as well very restricted. In fact, if the distribution of the data is not symmetric, replacing missing values with central tendency estimates such as the mean, the median or the mode will be incorrect and produce biased results even in presence of MCAR data  \citep[p. ~52]{raghunathan2015missing}. Additionally, some studies have found that the disadvantages of mean imputation are reduced with missingness rates below 10\% and low correlations between variables, however, in general and together with median and mode (modus) imputation for data with non-normal distributions all endure the same limitations and are not very popular methods for imputing missing data \citep{jadhav2019comparison}. 



\subsection{Multivariate Imputation by Chained Equations}

Starting as a solution to the problem of missing data in public-use data bases \textbf{Multiple Imputation (MI)} has become a popular method providing statistically valid results for scientific estimands.


Based on the fact that imputing just one value for a missing record is incorrect as it can't be assumed to be the real one, a better solution is to perform some good guesses for the missing value based on the available information to get some possible (plausible) option to replace the unknown. By repeating the process of "guessing" some times and combining these best guesses with the observed data, it is possible to obtain different versions of the complete dataset which will lead to new versions of complete data to perform subsequent analysis with measurable errors and variances while addressing for the uncertainty due to imputation \citep[p. ~77]{raghunathan2015missing}. 

Multivariate Imputation by Chained Equations - MICE \citep{van2011mice} is a multiple imputation algorithm capable of performing imputation in more than one variable. In order to explain the way the algorithm works, it is needed to introduce additional notation. As in multiple imputation, a set of columns are used as predictors for some others, lets introduce the notation $X_{-j}$ to denote the set of columns used as predictors of the column with missing entries $X_j$. And then as $m$ imputations are generated, each imputation is denoted by a superscript and a dot on top so, for example the $m$-th imputed version of column $j$ is denoted as: $\dot{Y}_j^m$.

Before diving into the details of MICE, it is needed to briefly introduce the main idea of a Gibbs Sampler. In short is a process in which considering a distribution $\mathbf{P}(Z) = \mathbf{P}(z_1, ..., z_M)$, with $Z$ being a matrix with $M$ variables, from which it is desired to sample and assuming a chosen initial state for the Markov chain, step by step the values of each variable are replaced by a value drawn from the distribution of such variable conditioned on the values of all the remaining variables. So, $z_i$ in step $t$ is replaced by a value drawn from the distribution in step $t-1$ $\mathbf{P}(z_i ~|~z_{-i})$, where $z_{-i}$ is the set of $z_1, ...,z_M$ without $z_i$. Then, the process is repeated by cycling through the $M$ variables in a particular order or by choosing the candidates to be updated randomly from a given distribution \citep{bishop2006pattern}. 

Algorithm \ref{alg:MICE} describes the process followed by MICE to impute the data iteratively. It begins by specifying an imputation model for each variable $j$. Then, in steps 2 to 4, the first version of a complete dataset is generated after imputing missing values by replacing them with drawn random values from $X_{obs,j }$ variable after variable. Then steps 5 to 11 describe the repeated sequence of Gibbs sampler iterations by conditioning each time on the most recently drawn values of all other variables \citep{van1999flexible}. 

An iteration is defined as the process of imputing once the missing data in all the variables $X_j$ so, in Algorithm \ref{alg:MICE} an iteration is each of the $t$'s in the loop defined between steps 5 to 11, repeated over $m$ iterations which in practice is usually set to be 5 or 10 \citep[p. ~120]{vanBuuren2018}. 

\begin{algorithm}[!h]
	\caption{MICE Algorithm, adapted from \citep[p. ~120]{vanBuuren2018}}\label{alg:MICE}
	\begin{algorithmic}[1]
		\Require Dataset $X = (X_{mis}, X_{obs})$ with $p$ and then also $R$.
		\Require $m$: number of imputations
		\State Specify an imputation model $\mathbf{P} (X_{mis,j} ~|~ X_{obs,j}, X_{-j}^t, R )$ for $X_j$ with $j = 1, 2, ..., p$.
		\For{$j = 1,2,..., p$}
			\State Impute missing entries in $X_j$ by random draws from $X_{obs,j}$ and store it as $\dot{X}_j^0$.
		\EndFor
		\For{$t = 1,2,..., m$}
			\For{$j = 1,2,...,p$}
				\State Define the currently complete data without $X_j$ as 
				$$\dot{X}_{-j}^t = (\dot{X}_{1}^t, ..., \dot{X}_{j-1}^t, \dot{X}_{j+1}^{t-1}, ..., \dot{X}_{p}^{t-1})$$
				\State Draw $\dot{\phi}_{j}^t \sim \mathbf{P} (\phi_{j}^t ~|~ X_{obs,j}, \dot{X}_{-j}^t, R)$
				\State Draw imputations $\dot{X}_{j}^t \sim \mathbf{P} (X_{mis,j} ~|~ X_{obs,j}, \dot{X}_{-j}^t, R, \dot{\phi}_{j}^t )$
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

After the imputations are performed (calculated in parallel), $m$ imputed datasets are available and then $m$ analyses are meant to be performed and then combined by pooling them into one final analysis including the uncertainty of the missing values coming from the multiple imputed datasets. In terms of convergence, even though the Gibbs sampler aims for convergence in distribution, and it is harder to achieve that convergence in value, experience shows that MICE needs fewer iterations than Markov Chains \citep{van1999flexible}. In fact, the number of iterations needed to get valid results are between 5 to 20 \citep[p. ~126]{vanBuuren2018}. 

But, now the question is, which are the models available to be chosen for the imputations defined in Step 1? In the following subsections 3 conditionally specified models implemented with MICE are described: Bayesian Linear Regression (\textrm{norm}), Predictive Mean Matching (\textrm{PMM}) and Random Forests (\textrm{RF}). 

 As MICE algorithm's is (over simplified) the imputation of missing data on a variable after variable basis and then repeat the process to get $m$ plausible option, it is easier and more intuitive to explain the first 2 imputation models in Univariate Setups (\textrm{norm} and \textrm{PMM}): that is, in a simple dataset where only one variable has missing entries. And then, such concepts are easily replicated one by one over all the variables $X_j$ with missing entries.

For this, keeping the notation proposed by \cite{vanBuuren2018} together with the one introduced in Section 2, let lower-case $x$ be a Univariate version of $X$ with incomplete data (so, only $x$ has missing values and therefore is the variable to be predicted) and the predictors of the model to be collected in $\mathcal{X}$ (note this is a collection of $n$ rows and $q < p$ complete parameters chosen to be the predictors of $x$). Then, $\mathcal{X}_{obs}$ is the subset with $n_1$ rows of $\mathcal{X}$ for which $x$ is observed and $\mathcal{X}_{mis}$ the remaining $n_0$ rows for which $x$ is missing. The $n_1$-vector with observed data in $x$ is $x_{obs}$ and the one with the missing data is $x_{mis}$ (with length $n_0$).

\subsubsection{Bayesian Linear Regression}
\label{ssec: norm}

The model is based on the normal linear model for prediction and improved by the addition of noise and uncertainty to the parameters of the predictive model calculated following a Bayesian approach: by drawing them from their posterior distribution. Thus, it can be described as:
\begin{equation}
	\label{eq:norm}
	\dot{x} = \dot{\beta_0} + \mathcal{X}_{mis} \dot{\beta_1} + \dot{\epsilon},
\end{equation}
where $\dot{\epsilon} \sim N(0, \dot{\sigma}^2)$ is the random noise term and $\dot{\beta_0},  \dot{\beta_1}$ and $\dot{\sigma}^2$ are random realisations from their posterior distribution given the data \citep[p. ~67]{vanBuuren2018}. 

Algorithm \ref{alg:norm} describes step by step the way to impute the missing data under the normal linear model as presented in Equation \eqref{eq:norm}. Starting from the vector of observed data $x_{obs}$, and the matrices of predictors with and without missing data in $x$ ($\mathcal{X}_{obs}$ and $\mathcal{X}_{mis}$, respectively), between steps 1 to 3 the estimates' coefficients $\hat{\beta}$ are calculated. Then, those are used to calculate the random realization for $\dot{\sigma}^2$ in step 5 adjusted by a random variable $\dot{g}$ drawn from a $\chi^2$ distribution with parameter $\nu = n_1-q$. After this, $q$ drawn values from $N(0,1)$ are stored in vector $\hat{z_1}$ followed by calculating the square root of $V$ from step 2 to then, in step 8, calculate the adjusted coefficients $\dot{\beta}$ from adding the coefficients obtained in 3 ($\hat{\beta}$) and the result of computing $\dot{\sigma}\dot{z_1}\sqrt[2]{V}$. With this result, just as with Step 6, a vector $\hat{z_2}$ is made from $n_0$ independent draws from a normal distribution with mean 0 and variance 1 which is then used in step 10 to calculate the new predicted values $\dot{x} = \mathcal{X}_{mis}\dot{\beta} + \dot{z_2}\dot{\sigma}$ to impute the missing ones. Please note the inclusion of $\kappa$ in step 2 to avoid singularity problems with matrices and it should have a positive value close to 0 \citep[p. ~68]{vanBuuren2018}.

\begin{algorithm}[H]
	\caption{Bayesian imputation under the normal linear model for a univariate setup, adapted from \citep[p. ~68]{vanBuuren2018}}\label{alg:norm}
	\begin{algorithmic}[1]
		\Require $x_{obs}$: $n_1 \times 1$ vector of observed data in the variable $x$ to be imputed.
		\Require $\mathcal{X}_{obs}$: $n_1 \times q$ matrix of predictors of rows with observed data in $x$. 
		\Require $\mathcal{X}_{mis}$: $n_0 \times q$ matrix of predictors of rows with missing data in $x$. 
		\State Calculate the cross-product matrix $S = \mathcal{X}'_{obs}\mathcal{X}_{obs}$.
		\State Calculate $V = (S + \textrm{diag}(S)\kappa)^{-1}$, with $\kappa$ small.
		\State Calculate the coefficients $\hat{\beta} = V  \mathcal{X}'_{obs} x_{obs}$.
		\State Draw a random variable $\dot{g} \sim \chi^2_\nu$ with $\nu = n_1 - q$.
		\State Calculate $\dot{\sigma}^2 = (x_{obs} - \mathcal{X}_{obs}\hat{\beta})' (x_{obs} -  \mathcal{X}_{obs}\hat{\beta})/\dot{g}$
		\State Draw $q$ independent $N(0,1)$ variates in vector $\dot{z_1}$.
		\State Calculate $\sqrt[2]{V}$ by Cholesky decomposition.
		\State Calculate $\dot{\beta} = \hat{\beta} + \dot{\sigma}\dot{z_1}\sqrt[2]{V}$.
		\State Draw $n_0$ independent $N(0,1)$ variates in vector $\dot{z_2}$.
		\State Calculate the $n_0$ values $\dot{x} = \mathcal{X}_{mis}\dot{\beta} + \dot{z_2}\dot{\sigma}$.
	\end{algorithmic}
\end{algorithm}

\subsubsection{Predictive Mean Matching}
\label{ssec:pmm}

According to the proposal for the Predictive Mean Matching (PMM) method made by \cite{little1988missing}, in a univariate setup where parameter $x$ is the one to impute, it will match each missing item $\langle x_{mis,i} \rangle$ to the item with the $d$-closest predictions from the observed ones $\langle x_{obs,i} \rangle$ and then use one among these $d$ observed values (in $x$) to impute the missing value. This final choice is drawn randomly.

The procedure for imputations following the Predictive Mean Matching algorithm is described in Algorithm \ref{alg:pmm}. It starts by calculating both the regression coefficients $\hat{\beta}$ and $\dot{\beta}$ following steps 1 to 8 from Algorithm \ref{alg:norm}. Then, in Step 2, it matches the predictions from the observed ($i^*$) and the missing ($j^*$) items by performing a so-called \textrm{Type 1 matching} (the default choice in the computational implementation) in which the "distances" $\dot{\eta}(i^*,j^*)$ between them are calculated. Done that, sets $Z_{j^*}$ with $d$ candidates (donors) are constructed from $\mathcal{X}_{obs}$ in a way in which they are the minimum for all the missing items $j^*$. then in step 4, one donor for each $Z_j^*$ is randomly drawn and set then in the final step to be the value chosen for the imputation of the missing one.  

\begin{algorithm}[H]
	\caption{Predictive mean matching in a univariate setup, taken and adapted from \citep[p. ~81]{vanBuuren2018}}\label{alg:pmm}
	\begin{algorithmic}[1]
		\Require $x_{obs}$: $n_1 \times 1$ vector of observed data in the variable $x$ to be imputed.
		\Require $\mathcal{X}_{obs}$: $n_1 \times q$ matrix of predictors of rows with observed data in $x$. 
		\Require $\mathcal{X}_{mis}$: $n_0 \times q$ matrix of predictors of rows with missing data in $x$.
		\Require $d$: number of donors.  
		\State Calculate $\dot{\beta}$ and $\hat{\beta}$ by following steps 1 to 8 of Algorithm \ref{alg:norm}.
		\State Calculate $\dot{\eta}(i^*,j^*) = | \mathcal{X}_{obs,i^*} \hat{\beta} -  \mathcal{X}_{mis,j^*} \dot{\beta}|$, with $i^* = 1, ..., n_1$ and $j^* = 1, ..., n_0$.
		\State Construct $n_0$ sets $Z_{j^*}$, each with $d$ candidate donors, from $\mathcal{X}_{obs}$ such that $\sum_d \dot{\eta}(i^*,j^*)$ is minimum for all $j^* = 1, ..., n_0$. Break ties randomly. 
		\State Draw randomly one donor $x_{i_{j^*}}$ from $Z_{j^*}$.
		\State Calculate imputations $\dot{x}_{j^*} = x_{i_{j^*}}$.
	\end{algorithmic}
\end{algorithm}

So, as PMM will impute only observed values, it is always predicting realistic values in the range of the data. Additionally, unlike the Bayesian Linear Regression there is no need to define an explicit model for the distribution of the missing values and still exhibits good performance even in presence of skewed data.  However, PMM has shown to decrease its quality in presence of small datasets and small choice of $d$ (sometimes leading to choosing the same donor for many imputations) or if the proportion of missing data generates imbalancements on it \citep{vanBuuren2018}. 

\subsubsection{Random Forest Imputations}
\label{ssec:micerf}

Up until this point, Bayesian Linear Regression and PMM  were mainly dealing with linear relations and were explained for datasets with only one feature having missing entries in order to make it understandable and extendable to multivariate missing setups just by repeating the process over the remaining possible features with missing entries. 

Now, in this (\ref{ssec:micerf}), \ref{ssec:missranger} and \ref{ssec:mixgb} sections,  we will explain the algorithms and methods with $X$ having one or more incomplete variables $X_j$. For this, we will refer to some subsets of the full dataset $X$ depending on how the missingness is present: if we refer to the observed values of feature $X_j$ being imputed as $X_{obs,j}$ and the missing entries in the same column as $X_{mis,j}$, when we refer to the remaining columns of the dataset $X_{obs,-j}$ it will be the subset from dataset $X$ with columns different than $X_j$ and with just the rows where feature $X_j$ has been observed ($r_{ij} = 1$) and respectively $X_{mis,-j}$ will be the columns from the dataset $X$ without $X_j$ with only the rows where $X_j$ is missing ($r_{ij} = 0$). Then, $X_{obs,-j}$ might have missing entries and $X_{mis,-j}$ could have observed values.

Thus, grounded on the Random Forests algorithm described in Section \ref{ssec:rf} and its flexibility to deal with multicollinearity and skewed distributions while being robust to outliers the imputation methods that we are going to be described in the following sections and subsections will benefit as well from such improvements as they all are Tree-based algorithms \citep[p. ~85]{vanBuuren2018}. 

Algorithm \ref{alg:micerf} follows the proposal made by \cite{doove2014recursive} to impute missing data through random forests and is implemented in the framework of MICE which along this report will be identified as \textrm{RF}. Please note it is described for just one imputation but the extension for multiple imputation can be made by repeating the process $m$ times. 
\begin{algorithm}[H]
	\caption{MICE RF (one imputation), adapted from \citep{doove2014recursive}}\label{alg:micerf}
	\begin{algorithmic}[1]
		\Require $X'$: $n \times p$ matrix of ordered predictors, i.e. with increasing amount of missing values per column. 
		\Require $\mathbf{B}$: number of bootstrap samples.
		\Require $L$: number of iterations.
			\For{$j = 1, 2, ..., p$} \Comment{$j$ goes over the sorted $p$ variables}
				\State Impute $\dot{X}_j^0$ by drawing random values from $X'_{obs,j}$ and store them in $\dot{X}$
			\EndFor
			\For{$l = 1,2, ...L$} 
			\State Create $X_{donors}=\{x_{donors,ij}\}$
			\For{$j = 1, 2, ..., p$} 
				\State Draw $\mathbf{B}$ bootstrap samples from $\dot{X}$, restricted to members in $X'_{obs,j}$ 
				\For{$b = 1, 2, ..., \mathbf{B}$}
					\State Fit a Random Forest on every $\dot{X_{b}}$ and store it as $T_b$.
					\State For each $x_{mis,ij}$ find the leaf from $T_b$ and store all the values in $\mathbb{d}$.
					\State Add $\mathbb{d}$ to the list of donors for the missing entry: $x_{donors,ij} = x_{donors,ij} \cup \mathbb{d}$.
				\EndFor
				\State For each $x_{mis,ij}$, draw randomly one value from $x_{donors,ij}$ and impute it in $\dot{X_j}$.
				\State Replace the new complete version of $\dot{X}_j$ in $\dot{X}$.
			\EndFor
		\EndFor
		\State Return the imputed matrix $\dot{X}$
	\end{algorithmic}
\end{algorithm}
\noindent In steps 1 to 3 is made the initial imputation of all the missing entries, column-wise, by drawing random values from the respective column feature. Then, for each iteration, a data structure $X_{donors}$ is created to store all the donors or possible values for the imputations of each missing entry $x_{mis,ij}$, but please bear in mind that each entry from $X_{donors}$ will store a list of possible values that will be updated (and increased) iteratively (Step 5) \footnote{To be more explicit, $X_{donors}$ could be a matrix in which all its entries $x_{ij}$ are lists that will contain the donors or candidates for the final imputations to be drawn from}. Done this, for each column the following cycle is made:  $\mathbf{B}$ bootstrap samples from the imputed matrix $\dot{X}$ are drawn but restricted to the observed values in $X_{obs}$ in order to train a Random Forest model from each bootstrapped set, resulting in $\mathbf{B}$ models after Step 9. Then in steps 10 and 11, for each missing entry is determined in which leaf it will end up according to the models $T_b$ to then take all the donors from these final leaves and get a full list of donors from all the bootstrapped models to be stored in the corresponding entry in $X_{donors}$. Done that, in step 13, one random value is drawn from all the listed donors for each missing entry and then after all are imputed, the new imputed version of the column is added to $\dot{X}$ in step 14. Done that, the cycle described between steps 5 to 15 are repeated $L$ times yielding to one final imputed dataset \citep{doove2014recursive}. 

\subsection{Imputation by Chained Random Forests}
\label{ssec:missranger}

Derived by the same principle of \textrm{RF} to be able to deal with mixed-type data and nonlinear distributions for multiple imputation of missing values, alternative implementations of it grounded on predictions made by Tree-Based and more precisely, Random Forests, are being found as additional options to impute the missing values. The proposal of \citep{stekhoven2012missforest} is known as \textrm{missForest} and its procedure is summarized in Algorithm \ref{alg:missForest} for one imputation ($m=1$). 

\begin{algorithm}[H]
	\caption{missForest (one imputation), taken and adapted from \citep{stekhoven2012missforest}}\label{alg:missForest}
	\begin{algorithmic}[1]
		\Require $X'$: $n \times p$ matrix of ordered predictors, i.e. with increasing amount of missing values per column. 
		\State Impute $X'$ and store it in $\dot{X}$ by a simple imputation model.
		\While{not $\gamma$}
		\For{$j = 1, 2, ..., p$} \Comment{$j$ goes over the sorted $p$ variables}
		\State Fit a Random Forest $f_j : X_{obs,j} \sim X_{obs,-j}$
		\State Predict $\hat{X_j}$ using $X_{mis}$, so: $\hat{X_j} = f_j(X_{mis})$
		\State Update $\dot{X}$ by replacing $\dot{X_j}$ by $\hat{X_j}$, so: $\dot{X_j} = \hat{X_j}$ 
		\EndFor
		\State Update $\gamma$
		\EndWhile
		\State return $\dot{X}$ 
	\end{algorithmic}
\end{algorithm}
\noindent First make sure $X$ is sorted column-wise with respect to the amount missing values in ascending order ($|X_{mis,j}| \leq |X_{mis,j+1}|$) and save it as $X'$. Then, perform a first guess imputation round of all the missing values by replacing them with a fast approach like naive imputation with mean or mode and store the imputed set as $\dot{X}$. Then, for each variable $p \in X'$ do one after another: Fit a random forest $f_j$ by training it to predict $X_{obs,j}$ based on the set of columns without feature $j$ so $X_{obs,-j}$ and then predict a new version of column $j$ from $f_j$ and name it $\hat{X_j}$. Done that, use $\hat{X_j}$ to replace the corresponding column into the Imputed set $\dot{X}$. Repeat the algorithm until the stopping criterion $\gamma$ is met and then return the last version of $\dot{X}$. 

The stopping criterion $\gamma$ in \textrm{missForest} is defined to be met when the difference between two consecutive versions of $\dot{X}$ from step 10 (denoted as $\dot{X}^{(s)}$ in step $s$ and $\dot{X}^{(s+1)}$ in the next step $s+1$) increases for the first time with respect to both Categorical and Numerical features according to the following definitions. If $\mathbb{C}$ is the set of Categorical variables and $\mathbb{N}$ is the set of Numerical variables in $X$, then $\gamma = \gamma_\mathbb{C} + \gamma_\mathbb{N}$ with:
\begin{equation}
	\gamma_\mathbb{C} = \frac{\sum_{j\in\mathbb{C}} \sum_{i \in n} \mathbb{1}_{\dot{x}_{mis,ij}^{(s+1)} \neq \dot{x}_{mis,ij}^{(s)}} }{|X_{mis,\mathbb{C}}|}
	\; \text{ and } \;
	\gamma_\mathbb{N} = \frac{\sum_{j\in\mathbb{N}} (\dot{x}_{mis,ij}^{(s+1)}-\dot{x}_{mis,ij}^{(s)})^2 }{\sum_{j\in\mathbb{N}} (\dot{x}_{mis,ij}^{(s+1)})^2} ,
\end{equation}
where $|X_{mis,\mathbb{C}}|$ is the number of missing entries in the categorical variables from $X$ and $\mathbb{1}_{\dot{X}^{(s+1)} \neq \dot{X}^{(s)}}$ is the indicator function taking value of $1$ when $\dot{x}_{mis,ij}^{(s+1)} \neq \dot{x}_{mis,ij}^{(s)}$ and $0$ when $\dot{x}_{mis,ij}^{(s+1)} = \dot{x}_{mis,ij}^{(s)}$ \citep{stekhoven2012missforest}.



\textrm{missRanger} is an implementation of imputation with Random Forests proposed by \cite{mayer2019missranger} which based on \textrm{missForest} (and among other additional computational optional enhancements), adds the option of predictive mean matching to it. That is, it allows to choose if when the model is fitted (so, in step 5 from Algorithm \ref{alg:missForest}) the candidates for new values to be used as predictions are drawn from the $d$ best possible candidate donors as in \textrm{PMM} (Algorithm \ref{alg:pmm}). Thus, all the imputed values will be always taken from the observed data while the variance in the resulting conditional distributions gets to a realistic level \citep{mayer2019missranger}. 
\\
\subsection{Multiple Imputation Through XGBoost}
\label{ssec:mixgb}



Just as with the implementation of multiple imputations based in Random Forests, \cite{deng2023multiple} proposed \textrm{mixgb}: a method to impute the missing values by using the XGBoost algorithm from \cite{chen2016xgboost}.
Just as with the implementation of multiple imputations based in Random Forests, \cite{deng2023multiple} proposed \textrm{mixgb}: a method to impute the missing values by using the XGBoost algorithm from \cite{chen2016xgboost}.
Just as in \textrm{missRanger}, the imputation has the option to include predictive mean matching and additionally subsampling. Which, according to the author, improve the variability of missing data while enhancing imputation quality \citep{deng2023multiple}.


When reviewed more in detail, \textrm{mixgb} has some options that can be chosen by the user and if needed: 
\begin{itemize}
	\item \textbf{Subsampling:} the ratio of the sample from the dataset can be varied (ratio $<1$) or left without subsampling (that is using the complete data so the ratio is left to be $1$). For this subsection, a subsample from $X$ is denoted as $X^*$. 
	\item \textbf{PMM Type:} offers 4 options according to how the models are trained and how the donors and the final imputed values are chosen from combining models trained from the whole data or from subsamples. To explain how \textrm{mixgb} works in predicting the missing values for a variable $X_j$, let  $\ddot{f}_j$ be the model trained with the whole data so $\ddot{f}_j: X_{obs,j} \sim X_{obs,-j}$. And $\tilde{f}_j^*$ be the model trained with subsampled versions from the whole data so $\tilde{f}_j^*: X_{obs,j}^* \sim X_{obs,-j}^*$. Then, following this notation, the relevant PMM options are:
	\begin{itemize}
		\item \textit{Type 1:} the predicted values for the donors are obtained by $\ddot{f}_j:$ and the predicted values to impute the missing data are produced by $\tilde{f}^*_j$.
		\item \textit{Type 2:} the predicted values for the donors and the predicted values to impute the missing data are both produced by $\tilde{f}^*_j$.
	\end{itemize}
\end{itemize}
\noindent Even when there are also Type 0 and Type 3 options, the first one is discarded as it will always uses the same model along the $m$ imputations ignoring variability between them and the Type 3 has a high computational cost as it needs 2 draws for each imputation. 


The detailed algorithm is described in Algorithm \ref{alg:mixgb}. Starting from the initial dataset $X$, first sort it column-wise from the feature with less missing entries to the one with the most and name it $X'$. Then, perform a simple imputation of all the missing entries in order to have the first version of a complete dataset $\dot{X}$. Now, if the matching PMM type chosen is 1, a new version of $\ddot{X}_{obs,j}$ is created by training $p$ XGBoost models fitted from a copy of $\dot{X}$ that will predict the values variable after variable (Steps 3 to 8). Done that, for each of the $m$ imputations is performed the following process $S$ times: a subsample from $\dot{X}$ is made and stored as $X^{(s)*}$ which is then used to fit an XGBoost model $\tilde{f}^*_j$ for each variable. 

Done that, this model is used to predict $\tilde{X}^*_{mis,j}$ from $X_{mis,-j}$. Now, depending on the PMM type, there are 3 options:
\begin{itemize}
	\item \textbf{Type 1:} Match $\ddot{X}_{obs,j}$ to $\tilde{X}^*_{mis,j}$ to get the donor(s) and update $X^{(s)}$.
	\item \textbf{Type 2:} Predict  $\tilde{X}^*_{obs,j}$ from $X_{obs,-j}$ and match the results to $\tilde{X}^*_{mis,j}$ to get the donor(s) and update $X^{(s)}$.
	\item For any other case (this is the default choice for categorical data), use $\tilde{X}^*_{mis,j}$ to update $X^{(s)}$.
\end{itemize}
And finally, before returning the updated version of the dataset in the last step ($X^{(S)}$), reorder the variables to match the initial one from $X$. 

\begin{algorithm}[H]
	\caption{mixgb ($m$ imputations), taken and adapted from \citep{deng2023multiple}}\label{alg:mixgb}
	\begin{algorithmic}[1]
		\Require $X$: $n \times p$ matrix of data with missing entries.
		\Require $pmm.type$ : Type of pmm chosen for the imputation.
		\Require $m$: Number of Imputations
		\Require $S$: Number of Iterations
		\State Order $X$'s predictors to have increasing an amount of missing values per column and store it as $X'$.
		\State Impute $X'$ and store it in $\dot{X}$ by a simple imputation method.
		\If{$pmm.type = 1$}
		\State $X = \dot{X}$
		\For{$j = 1, 2, ..., p$} \Comment{$j$ goes over the sorted $p$ variables}
		\State Fit an XGBoost model $\ddot{f}_j : X_{obs,j} \sim X_{obs,-j}$.
		\State Predict $\ddot{X}_{obs,j} = \ddot{f_j}(X_{obs,-j})$
		\EndFor
		\EndIf
		\For{$t = 1, 2, ..., m$}		
		\State $X^0 = \dot{X}$
		\For{$s = 1, 2, ..., S$}
		\State $X^{(s)} = X^{(s-1)}$
		\State Subsample $X^{(s)}$ and save it as $X^{(s)*}$
		\For{$j = 1, 2, ..., p$} \Comment{$j$ goes over the sorted $p$ variables}
		\State Fit an XGBoost model $\tilde{f}^*_j : X^{(s)*}_{obs,j} \sim X^{(s)*}_{obs,-j}$.
		\State Predict $\tilde{X}^*_{mis,j} = \tilde{f}^*_j(X_{mis,-j})$
		\If{$pmm.type=1$}
		\State Update $X^{(s)}$ with donors from $X_{obs,j}$ by matching $\tilde{X}^*_{mis,j}$ to $\ddot{X}_{obs,j}$
		\ElsIf{$pmm.type=2$}
		\State Predict $\tilde{X}^*_{obs,j} =\tilde{f}^*_j (X_{obs,-j})$
		\State Update $X^{(s)}$ with donors from $X_{obs,j}$ by matching $\tilde{X}^*_{mis,j}$ to $\tilde{X}^*_{obs,j}$
		\Else
		\State Update $X^{(s)}$ with $\tilde{X}^*_{mis,j}$.
		\EndIf
		\EndFor
		\EndFor
		\State Reorder the variables of $X^{(S)}$ and return it.
		\EndFor
		\State Return the $m$ imputed datasets. 
	\end{algorithmic}
\end{algorithm}



\subsection{Imputation Metrics}

Given the variety of methods used for imputation, it is important to set a common metric to measure their performance. Starting from the complete dataset without missing values $X^{true}$, the first 2 metrics (\textbf{IPM} and \textbf{NRMSE}) are measures of accuracy and are meant to calculate how close are the values in the imputed dataset $X^{imp}$ to the true ones in the original dataset before removing the data. 

Done that, the correlations before and after imputation are also used to investigate how they differ from each other by measuring the distance between the mean of the correlations in the original dataset before removing any data and the mean of the correlations of the imputed datasets.

Said that, we can proceed with the detailed calculation of each metric. 


\subsubsection{NRMSE}

The Normalized Root Mean Squared Error is a measure of distance for numeric variables that computes the squared root from the MSE metric introduced in Equation \eqref{eq:mse} and then normalizes such results in order to make fair comparisons in presence of the different scales among the variables in the dataset \citep{jadhav2019comparison}. The full equation in terms of imputed and true values is, as presented by \cite{ramosaj2022relation}:
\begin{equation}
	\label{eq:rmse}
	NRMSE = \frac{\sqrt{\sum_{{i,j} \in X^{mis}}  \big(x^{imp}_{ij} - x^{true}_{ij} \big)^2 } } { \sqrt{\sum_{{i,j} \in X^{mis}} \big(x^{imp}_{ij} - \bar{x}^{mis}_{ij} \big)^2 } },
\end{equation}
where $\bar{x}^{mis}_{ij}$ is the mean of the true values for which there was a value missing in the amputed version of $X^{true}$: so, the mean of the sequence $\{x^{true}_{ij}:r_{ij}=0\}$. Then, as a measure of error, the closer its value is to 0, the better the imputation method performance will be.

\subsubsection{IPM}

Proposed by \cite{suh2023comparison} it is meant to summarize in one single metric the distance between $X^{true}$ and $X^{imp}$ for both numerical and categorical variables. Let the distance between two numeric columns $j$ of $X^{true}$ and $X^{imp}$ as 
\begin{equation}
	\delta \big( x_{ij}^{true} - x_{ij}^{imp}\big) = \frac{|x_{ij}^{true} - x_{ij}^{imp}|}{ \max (x_{j}^{true},x_{j}^{imp}) - \min (x_{j}^{true},x_{j}^{imp}) }
\end{equation}
and analogously the distance between two categorical columns $j$ of $X^{true}$ and $X^{imp}$ as
\begin{equation}
	\delta \big( x_{ij}^{true} - x_{ij}^{imp}\big) = \mathds{1} \big(x_{ij}^{true} \neq x_{ij}^{imp} \big),
\end{equation}
where $\mathds{1}(\cdot)$ is 1 if $x_{ij}^{true} \neq x_{ij}^{imp}$ are different and 0 if they are equal. Then IPM is defined as
\begin{equation}
	IPM = \sum_{i=1}^n \sum_{j=1}^p \frac{\delta \big( x_{ij}^{true} - x_{ij}^{imp}\big)} {n^{mis}},
\end{equation}
and, just as with NRMSE the lower the value for IPM, the closer the imputed dataset $X^{imp}$ is to the true one $X^{true}$ and the better the imputation performance will be. 

\subsubsection{Correlation Distances}

Correlation is the measure of \textbf{linear} relationship between 2 variables $U$ and $V$ both with the same lengths ($|U|=|V|$) and is defined mathematically to be for the Pearson case:
\begin{equation}
	\mathbb{r}_{Pe}(U,V) = \frac{\sum_{i \in |U|} \big(u_i - \bar{U} \big) \big(v_i - \bar{V} \big)} { \sqrt{\sum_{i \in |U|} \big(u_i - \bar{U} \big)^2 } \sqrt{\sum_{i \in |U|} \big(v_i - \bar{V} \big)^2 }},
\end{equation}
where $\bar{U}$ and $\bar{V}$ are the means of each variable and is meant to indicate which kind of linear relationship exists between the variables being compared. Due to its mathematical nature, the resulting values can vary between -1 and 1. If its value is positive, will be indicator of a directly proportional relation of the variables, meaning if one variable increases the other one as well and if one decreases the other one as well, linearly. But, when negative, will be indicator of an inverse relation meaning that if one variable increases the other decreases, linearly. And, if $\mathbb{r}$ is close to 0, it will be representative of either non-linear or a very weak linear relationship while when it gets closer to either +1 or -1 will be indicator of a strong linear relationship between $U$ and $V$ \citep{xiao2016using}. 

Similarly, the Spearman coefficient is defined to be:
\begin{equation}
	\mathbb{r}_{Sp}(U,V) = 1 - \frac{ 6 \sum_{i \in |U|} \big(u'_i - y'_i \big)^2 } { |U| \big(|U|^2-1\big)},
\end{equation}
where $u'_i$ and $v'_i$ are the paired ranked variables and then for this case, the linear relationship is dropped being able to explain mainly the monotonicity between the variables under comparison and being more robust and statistically valid for non-normally distributed variables. In terms of its values, they fall into the same range between -1 and +1 as in the Pearson correlations and also mean a stronger relationship when the resulting value departs from 0 \citep{xiao2016using}. 

Now, in order to compare the imputations, the resulting correlation coefficients for each imputation method ($X^{imp}$) are compared to the ones presented in the initial complete dataset ($X^{true}$) by measuring 3 distances between the resulting correlation matrices. The chosen ones are defined in general for any 2 matrices $A=[a_{i'j'}],B=[b_{i'j'}] \in \mathsf{R}^{m' \times n'}$ with  $i'=1,2,...,m'$ and $j'=1,2,...,n'$ as follows:
\begin{itemize}
	\item \textbf{MAE:} the mean absolute error is: 
	\begin{equation}
		MAE = \frac{ \sum_{i'=1}^{m'} \sum_{j'=1}^{n'} ||a_{i'j'} - b_{i'j'}|| } {m' \cdot n'},
	\end{equation}
	where $|| \cdot ||$ is the notation of the absolute value \citep{hodson2022root}.
	\item \textbf{RMSE:} the root mean squared error is as presented by \citep{hodson2022root}:
	\begin{equation}
		RMSE = \sqrt{ \frac{ \sum_{i'=1}^{m'} \sum_{j'=1}^{n'} (a_{i'j'} - b_{i'j'})^2 }{m' \cdot n'} },
	\end{equation}
	\item \textbf{Frobenius:} the Frobenius distance is:
	\begin{equation}
		\mathbb{F} = \sqrt{ \sum_{i'=1}^{m'} \sum_{j'=1}^{n'} ||a_{i'j'} - b_{i'j'}||^2  },
	\end{equation}
	where $|| \cdot ||$ is the notation of the absolute value \citep[p. ~ 55]{van1983matrix}.
\end{itemize}
\noindent So, in an ideal scenario if the 2 correlation matrices are identical these calculated distances would have a value of 0 and the more they increase, the bigger the distance between them will be. 
\\

\subsection{Feature Selection and Multiple Imputation}
\label{ssec:micefeatsel}

As after performing multiple imputation, there will be 5 imputed datasets with 5 possible best models, each with a different set of best features being selected, it is needed to decide which are the best ones among these sets. So, following an approach which could be understood as the pooling version for other metrics but applied for feature selection after multiple imputation, a proposal using frequency of non-zero regression coefficients is made as suggested by \cite{zahid2020variable} : 
\begin{equation}
	\text{select} \, X_j, \quad \text{if} \quad \frac{\sum_{t=1}^m \mathbb{1}(X_{j,m} \text{ is chosen})}{m} \geq \delta,
\end{equation}
where $\mathbb{1}(X_{j,m} \text{ is chosen})$ is a function counting how many times the feature $X_j$ is chosen for iteration $m$. Thus, it will select the feature if among the possible $m$ models it is chosen in a proportion that is greater or equal than $\delta$. 

\fi



\iffalse
\section{Results}
\subsection{Training Times}

\subsubsection{Baseline Training Times}

Having reviewed the MSE results, it is worth reviewing as well the average computational times to tune the models and the effect the imputations might have into it. To be precise, the time being recorded is the average time to train one model with one of the hyperparameters’ combination according to the defined grid. So, said that and to set a benchmark again, the tuning times for the complete models before amputation and imputation were recorded and are shown in Table \ref{tab:MSEbase_times}. 

\begin{table}[H]
	\caption{Summary Statistics for the Training time in minutes for the Complete Dataset} \label{tab:MSEbase_times}
	\centering
	\small
	\begin{tabulary}{\textwidth}{lccccccc}  
		\toprule[2 pt]
		\textbf{ML Method} & \textbf{Min} & \textbf{1st. Qu.} & \textbf{Median} & \textbf{Mean} & \textbf{3rd. Qu.} & \textbf{Max} & \textbf{SD}\\
		\midrule
		\textrm{regr.cv\_glmnet} & 0.013 & 0.019 & \textbf{0.023} & 0.022 & 0.025 & 0.034 & 0.004 \\ 
		\textrm{regr.ranger} & 0.029 & 0.072 & \textbf{0.102} & 0.111 & 0.142 & 0.268 & 0.048 \\ 
		\textrm{regr.xgboost} & 0.009 & 0.030 & \textbf{0.049} & 0.066 & 0.090 & 0.290 & 0.048 \\ 
		\bottomrule[2 pt]
	\end{tabulary}
\end{table}
\noindent Here the results are different to the MSE, that is, the Lasso Penalized Linear Model was the fastest one with a median of 0.023 minutes, followed by the XGBoost with 0.049 minutes and finally Random Forests with 0.102 minutes.

\subsubsection{Training Times Results in comparison}

Figure \ref{fig:MSE_times} has depicted the average training times per imputation and ML Regression method. Just as with the MSE results, the horizontal lines are illustrative of the medians obtained for the baseline scenario for each ML Method and the color conventions are maintained as in the plot's legend. 

In this case, most of the medians are close to the horizontal lines showing that the imputation method is not affecting notoriously the time to train the ML Models for Regression. In any case, the most relevant result is that the variances in the results for Random Forests (the range of the times obtained) seem to be more sensitive to the imputation model as the height of the boxplots for these cases are the biggest ones; being more visible for the cases in which the missing data was imputed following \textrm{norm} and \textrm{missRanger0} methods, but with lower variances at the 2 highest missingness rates for the last 2 mentioned methods.

\begin{figure}[H]
	\centering
	\caption{Tuning Times for each Regression Method and Missingness Rate. The horizontal Lines are the Median of the MSE's obtained for the Complete Dataset}
	\label{fig:MSE_times}
	\includegraphics[width = \textwidth]{Pictures/R_MLTimes.png}
\end{figure}

\fi


\iffalse
\subsubsection{Imputation Time}

With regard to the imputation times, before jumping into the results lets just recall that \textrm{listwise} deletion is not included here as even though it is the fastest to be computed, there is no real imputation being made and then no fair comparison to the other methods. Additionally, it is also worth mentioning that the times discussed in this subsection are the average times to get a fully imputed dataset. That is, for the multiple imputation methods, it is calculated as the time (in minutes) elapsed to perform the $m=5$ imputations divided by the number of imputations.

In Figure \ref{fig:impTime} are registered the imputation times for all the methods chosen. The fastest results are the ones for \textrm{norm} and \textrm{pmm}, with the first one having some more outliers for 10\% and 30\% missingness rates. The next faster is \textrm{mixGB} followed by \textrm{RF}. All these have medians below 2 minutes. On the other hand, the methods requiring more execution times were all the cases of \textrm{missRanger} where more than 2.5 minutes were needed and for some cases even more than 6 minutes.

\begin{figure}[H]
	\centering
	\caption{Imputation time in Minutes. Here is shown the average for $m=1$}
	\label{fig:impTime}
	\includegraphics[width = 0.7\textwidth]{Pictures/R_Imptime.png}
\end{figure}

\noindent Additionally, there is a common pattern for all the imputation methods with regards to the amount of missing data: the fastest one to be computed is always the one with 50\% missingness, followed by the one with 70\%, then 30\% and finally the case with just 10\% missing data.
\\
\fi 

